Outlier-aware Inlier Modeling and Multi-scale Scoring for Anomalous Sound Detection via Multitask Learning

This paper proposes an approach for anomalous sound detection that incorporates outlier exposure and inlier modeling within a unified framework by multitask learning. While outlier exposure-based methods can extract features efficiently, it is not robust. Inlier modeling is good at generating robust features, but the features are not very effective. Recently, serial approaches are proposed to combine these two methods, but it still requires a separate training step for normal data modeling. To overcome these limitations, we use multitask learning to train a conformer-based encoder for outlier-aware inlier modeling. Moreover, our approach provides multi-scale scores for detecting anomalies. Experimental results on the MIMII and DCASE 2020 task 2 datasets show that our approach outperforms state-of-the-art single-model systems and achieves comparable results with top-ranked multi-system ensembles.

==> bibtempl.tex <==
@article{Davis80-COP,
	Author = {Steven B. Davis and Paul Mermelstein},
	Journal = {IEEE Transactions on Acoustics, Speech and Signal Processing},
	Number = {4},
	Pages = {357--366},
	Title = {Comparison of Parametric Representations for Monosyllabic Word Recognition in Continuously Spoken Sentences},
	Volume = {28},
  Month = aug,
	Year = {1980}}

@article{Rabiner89-ATO,
	Author = {Lawrence R. Rabiner},
	Journal = {Proceedings of the IEEE},
	Number = {2},
	Pages = {257--286},
	Title = {A Tutorial on Hidden {Markov} Models and Selected Applications in Speech Recognition},
	Volume = {77},
  Month = feb,
	Year = {1989}}

@book{Hastie09-TEO,
	Address = {New York},
	Author = {Trevor Hastie and Robert Tibshirani and Jerome Friedman},
	Publisher = {Springer},
	Title = {The Elements of Statistical Learning -- Data Mining, Inference, and Prediction},
	Year = {2009}}

@inproceedings{Smith22-XXX,
	Author = {Jane Smith and Firstname2 Lastname2 and Firstname3 Lastname3},
	Pages = {100--104},
	Title = {A really good paper about {D}ymanic {T}ime {W}arping},
 	Booktitle = {Proc. {INTERSPEECH} 2022 -- 23\textsuperscript{rd} Annual Conference of the International Speech Communication Association},
    Address = {{Incheon, Korea}},
    Month = {{Sep.}},
	Year = {2022}}

 % use the Crossref field to copy any unspecified fields (such as booktitle) from another entry, 
@inproceedings{Jones22-XXX,
	Author = {Robert Jones and Firstname2 Lastname2 and Firstname3 Lastname3},
	Crossref = {Smith22-XXX},
	Pages = {105--109},
	Title = {An excellent paper introducing the {ABC} toolkit}}

@inproceedings{moore19_interspeech,
  author={Roger K. Moore and Lucy Skidmore},
  title={On the Use/Misuse of the Term {`Phoneme'}},
    Address = {{Graz, Austria}},
    Month = {{Sep.}},
  year=2019,
 	Booktitle = {Proc. {INTERSPEECH} 2019 -- 20\textsuperscript{th} Annual Conference of the International Speech Communication Association},
  pages={2340--2344},
  doi={10.21437/Interspeech.2019-2711}
}
